Generating Narrative Text in a Switching Dynamical System

Early work on narrative modeling used explicit plans and goals to generate stories, but the language generation itself was restricted and inflexible. Modern methods use language models for more robust generation, but often lack an explicit representation of the scaffolding and dynamics that guide a coherent narrative. This paper introduces a new model that integrates explicit narrative structure with neural language models, formalizing narrative modeling as a Switching Linear Dynamical System (SLDS). A SLDS is a dynamical system in which the latent dynamics of the system (i.e. how the state vector transforms over time) is controlled by top-level discrete switching variables. The switching variables represent narrative structure (e.g., sentiment or discourse states), while the latent state vector encodes information on the current state of the narrative. This probabilistic formulation allows us to control generation, and can be learned in a semi-supervised fashion using both labeled and unlabeled data. Additionally, we derive a Gibbs sampler for our model that can fill in arbitrary parts of the narrative, guided by the switching variables. Our filled-in (English language) narratives outperform several baselines on both automatic and human evaluations.

==> junk.tex <==
% Middle Three missing
 My roommate made fish for dinner last night .
 It was very difficult to get out of the house .
 The next day we went to the store and complained .
 The manager told me the food was terrible .
 I suggested he apply to for a cook 's position where I worked .

 Billy really needed help with his test .
 He decided to pull an all - nighter .
 The next day , he was ready to go to school .
 On the day of the test he arrived .
 Billy failed the test .

 Yesterday my friend and I got into a fight .
 The argument was about to fight and we lost our temper
 My friend and I fought for the fight and we went to the hospital .
 The doctor was very nice and we were okay .
 I 'm having her over for tea later this week .

Sally is a writer .
 Her writing is not great .
 She wrote a story about her life .
 The story was very bad .
 Sally failed in her efforts to complete the assignment .

 Tom rolled his wagon .
 His dad was driving down the hill .
 He accidentally hit the wagon .
 Tom 's dad flipped over the handlebars .
 Tom 's dad was not helpful ever .

 Tim was always on his bike during the summer .
 He had a lot of fun .
 One day he decided to cut his bike down .
 He hit a rock and fell off the bike and hit a tree .
 He broke his arm .


%Second and fourth missing

 <sos> Dorothy had just turned ninety years old on Friday . <eos>
 <sos> Her parents were coming to visit . <eos>
 <sos> Friends and family came from all around . <eos>
 <sos> On the day of the trip , she hugged her parents . <eos>
 <sos> She had a wonderfully exhausting day visiting with friends and family ! <eos>

 <sos> Ben has always wanted to learn how to play the piano . <eos>
 <sos> His parents bought him one . <eos>
 <sos> Ben enrolls in a piano class with a local tutor . <eos>
 <sos> Ben practiced every day . <eos>
 <sos> He gets better with every lesson . <eos>

%First and Second missing

 <sos> Mark has been working hard all week . <eos>
 <sos> He calls his boss to let him know he does n't know . <eos>
 <sos> Finally , they gave him leave to visit his family . <eos>
 <sos> He got on the plane really excited . <eos>
 <sos> His family were waiting for him at the airport and welcomed him home . <eos>


 <sos> Last week I had an idea . <eos>
 <sos> I was so nervous that I decided to make a presentation . <eos>
 <sos> I soon found it hard to come up with new ideas . <eos>
 <sos> I did n't think it would be so hard . <eos>
 <sos> But then , an idea came to me and I was back on track . <eos>
 
 Susie entered the school . <eos>
 <sos> She walked into the classroom . <eos>
 <sos> She explained to her teachers about her mistake . <eos>
 <sos> All of them believed her and said she could turn it in a day late . <eos>
 <sos> Thankfully , later that day she saw it was right where she had left it . <eos>

<sos> I had a bad relationship with my girlfriend . <eos>
 <sos> She was very upset and told me she was pregnant . <eos>
 <sos> Rachel told her family and it was very difficult . <eos>
 <sos> They all cried . <eos>
 <sos> They agreed that on the whole , it was good news . <eos>

\textcolor{gray}{Yesterday I was at the mall shopping.} & \textcolor{gray}{Ed was playing baseball in his yard.} \\
Suddenly, a man in a mask appeared. & He was running down the hill.\\
The man was walking around and he was gone. & His ball was coming towards him.\\
 He had to call me to help me get out of the store.& It was very scary!\\
\textcolor{gray}{I heard on the news that night they sent the UNK to prison.} & \textcolor{gray}{Ed was scared.} \\
